Proceedings of the Young Researchers Workshop on Positivity in Lie Groups

These notes transcribe a workshop about the notion of total positivity and $\Theta$-positivity and its relation to Higher Teichm\"uller Theory. $\Theta$-positivity is a notion of positivity in semisimple Lie groups and was recently introduced by Guichard and Wienhard as a generalization of Lusztig's total positivity. It is believed to be the cathartic notion to classify higher Teichm\"uller spaces. Without doubt, substantial progress will be achieved in the near future on the study of $\Theta$-positive structures. These notes provide an account of the state of the art as of 2021.

==> preface.tex <==
\thispagestyle{empty}

\chapter*{Preface}
\addcontentsline{toc}{chapter}{Preface}

Anna writes something ?
